Hermite Polynomial Features for Private Data Generation

Kernel mean embedding is a useful tool to represent and compare probability measures. Despite its usefulness, kernel mean embedding considers infinite-dimensional features, which are challenging to handle in the context of differentially private data generation. A recent work proposes to approximate the kernel mean embedding of data distribution using finite-dimensional random features, which yields analytically tractable sensitivity. However, the number of required random features is excessively high, often ten thousand to a hundred thousand, which worsens the privacy-accuracy trade-off. To improve the trade-off, we propose to replace random features with Hermite polynomial features. Unlike the random features, the Hermite polynomial features are ordered, where the features at the low orders contain more information on the distribution than those at the high orders. Hence, a relatively low order of Hermite polynomial features can more accurately approximate the mean embedding of the data distribution compared to a significantly higher number of random features. As demonstrated on several tabular and image datasets, Hermite polynomial features seem better suited for private data generation than random Fourier features.

==> tables/table_discrete_tab_hyperparams.tex <==

\begin{table}
\caption{Hyperparameters for discrete tabular datasets}
\label{tab:discete_hyper}
\vskip 0.2cm
\centering
\begin{NiceTabular}{ccccccc}
\toprule
& privacy & batch rate & order hermite prod & prod dimension & gamma & order hermite \\ \midrule
\Block{2-1}<\rotate>{\small Adult}
% &$\varepsilon=1$.0 & 0.1 & 5 & 7 & 1 & 100 \\
&$\varepsilon=0.3$ & 0.1 & 10 & 5 & 1 & 100 \\
&$\varepsilon=0.1$ & 0.1 & 5 & 7 & 1 & 100 \\ \midrule
\Block{2-1}<\rotate>{\small Census}
% &$\varepsilon=1.0$ & 0.01 & 10 & 5 & 0.1 & 100 \\
&$\varepsilon=0.3$ & 0.01 & 5 & 7 & 0.1 & 100 \\
&$\varepsilon=0.1$ & 0.01 & 5 & 7 & 0.1 & 100 \\
\bottomrule
\end{NiceTabular} 
\end{table}
